Coverage-Based Debloating for Java Bytecode

Software bloat is code that is packaged in an application but is actually not necessary to run the application. The presence of software bloat is an issue for security, for performance, and for maintenance. In this paper, we introduce a novel technique for debloating, which we call coverage-based debloating. We implement the technique for one single language: Java bytecode. We leverage a combination of state-of-the-art Java bytecode coverage tools to precisely capture what parts of a project and its dependencies are used when running with a specific workload. Then, we automatically remove the parts that are not covered, in order to generate a debloated version of the project. We succeed to debloat 211 library versions from a dataset of 94 unique open-source Java libraries. The debloated versions are syntactically correct and preserve their original behavior according to the workload. Our results indicate that 68.3% of the libraries' bytecode and 20.3% of their total dependencies can be removed through coverage-based debloating. For the first time in the literature on software debloating, we assess the utility of debloated libraries with respect to client applications that reuse them. We select 988 client projects that either have a direct reference to the debloated library in their source code or which test suite covers at least one class of the libraries that we debloat. Our results show that 81.5% of the clients, with at least one test that uses the library, successfully compile and pass their test suite when the original library is replaced by its debloated version.

==> abbrev.tex <==
%\usepackage{soul}
%\usepackage{tikz}

\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\makeatletter

\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}


==> app.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, xleftmargin=3.5ex, caption={A Java application that uses the Apache \texttt{commons-configuration2} library to get access to a configuration file. The application calls different methods in the library to handle a \texttt{Properties} or JSON file. For an user providing a \texttt{Properties} file, the code with green background is used code.}, label={lst:app},belowskip=-6\baselineskip]
import org.apache.commons.configuration2.*;
import org.apache.commons.configuration2.builder.*;
import org.apache.commons.configuration2.builder.fluent.*;

public class App {
 public static void main(String[] args) {
£  if(args[0].equals("-properties")) {£
£     Configurations configs = new Configurations();£
£     Configuration config = configs.properties(new File(args[1]));£
£     . . .£
   } else if (args[0].equals("-json")) {
     Parameters params = new Parameters();
     FileBasedConfigurationBuilder<JSONConfiguration> builder =
      new FileBasedConfigurationBuilder<>(JSONConfiguration.class)
          .configure(params.hierarchical()
            .setFileName(args[1]));
     JSONConfiguration config = builder.getConfiguration();
     . . . 
   } 
. . .
\end{lstlisting}

==> biographies.tex <==
\newpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/cesar.jpg}}]{C\'esar Soto-Valero}
is a PhD student in Software Engineering at KTH Royal Institute of Technology, Sweden. His research work focuses on leveraging static and dynamic program analysis techniques to mitigate software bloat. C\'esar received his MSc degree and BSc degree in Computer Science from Universidad Central ``Marta Abreu" de Las Villas, Cuba.
\end{IEEEbiography}
\vspace{-10.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/thomas.jpg}}]{Thomas Durieux}
is a Post-doc at KTH Royal Institute of Technology, Sweden. He is currently working on software debloat and software art. Thomas did his PhD on automatic program repair, with a specific focus on the production environment at INRIA Lille, France. 
\end{IEEEbiography}
\vspace{-10.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/nicolas.jpg}}]{Nicolas Harrand}
is a PhD student in Software Engineering at KTH Royal Institute of Technology, Sweden. His current research is focused on automatic software diversification. Nicolas studied Computer Science and Applied Mathematics in Grenoble, France.
\end{IEEEbiography}
\vspace{-10.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/benoit.jpg}}]{Benoit Baudry}
is a Professor in Software Technology at KTH Royal Institute of Technology in Stockholm, Sweden. He received his PhD in 2003 from the University of Rennes and was a research scientist at INRIA from 2004 to  2017. His research is in the area of software testing, code analysis and automatic diversification. He has led the largest research group in software engineering at INRIA, as well as collaborative projects funded by the European Union, and software companies.
\end{IEEEbiography}

==> er.tex <==
% code for "one to omany", etc. is taken from https://tex.stackexchange.com/q/141797/101651
\makeatletter
\pgfarrowsdeclare{crow's foot}{crow's foot}
{
    \pgfarrowsleftextend{+-.5\pgflinewidth}%
    \pgfarrowsrightextend{+.5\pgflinewidth}%
}
{
    \pgfutil@tempdima=0.6pt%
    \pgfsetdash{}{+0pt}%
    \pgfsetmiterjoin%
    \pgfpathmoveto{\pgfqpoint{0pt}{-9\pgfutil@tempdima}}%
    \pgfpathlineto{\pgfqpoint{-13\pgfutil@tempdima}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{9\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{-8pt}{-6pt}}% 
    \pgfpathlineto{\pgfqpoint{-8pt}{-6pt}}%  
    \pgfpathlineto{\pgfqpoint{-8pt}{6pt}}% 
    \pgfusepathqstroke%
}

\pgfarrowsdeclare{omany}{omany}
{
    \pgfarrowsleftextend{+-.5\pgflinewidth}%
    \pgfarrowsrightextend{+.5\pgflinewidth}%
}
{
    \pgfutil@tempdima=0.6pt%
    \pgfsetdash{}{+0pt}%
    \pgfsetmiterjoin%
    \pgfpathmoveto{\pgfqpoint{0pt}{-9\pgfutil@tempdima}}%
    \pgfpathlineto{\pgfqpoint{-13\pgfutil@tempdima}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{9\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%  
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{-6pt}{-6pt}}% 
    \pgfusepathqstroke%
    \pgfsetfillcolor{white}
    \pgfpathcircle{\pgfpoint{-11.5pt}{0}} {3.5pt}
    \pgfusepathqfillstroke%
}

\pgfarrowsdeclare{one}{one}
{
    \pgfarrowsleftextend{+-.5\pgflinewidth}%
    \pgfarrowsrightextend{+.5\pgflinewidth}%
}
{
    \pgfutil@tempdima=0.6pt%
    \pgfsetdash{}{+0pt}%
    \pgfsetmiterjoin%
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{-6pt}{-6pt}}% 
    \pgfpathlineto{\pgfqpoint{-6pt}{-6pt}}%  
    \pgfpathlineto{\pgfqpoint{-6pt}{6pt}}% 
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{-8pt}{-6pt}}% 
    \pgfpathlineto{\pgfqpoint{-8pt}{-6pt}}%  
    \pgfpathlineto{\pgfqpoint{-8pt}{6pt}}%    
    \pgfusepathqstroke%
}

\pgfarrowsdeclare{oone}{oone}
{
    \pgfarrowsleftextend{+-.5\pgflinewidth}%
    \pgfarrowsrightextend{+.5\pgflinewidth}%
}
{
    \pgfutil@tempdima=0.6pt%
    %\advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfsetdash{}{+0pt}%
    \pgfsetmiterjoin%
     \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \
    pgfpathmoveto{\pgfqpoint{-4pt}{-6pt}}% 
    \pgfpathlineto{\pgfqpoint{-4pt}{-6pt}}%  
    \pgfpathlineto{\pgfqpoint{-4pt}{6pt}}% 
    \pgfsetfillcolor{white}
    \pgfpathcircle{\pgfpoint{-11.5pt}{0}} {3.5pt}
    \pgfusepathqfillstroke%
}
\makeatother

\tikzset{%
    mylabel/.style={font=\footnotesize},
    pics/entity/.style n args={3}{code={%
        \node[draw,
        rectangle split,
        rectangle split parts=2,
        text height=1.5ex,
        text width=7em,
        text centered
        ] (#1)
        {#2 \nodepart[font=\small, text centered]{second}
            \begin{tabular}{>{\raggedright\arraybackslash}p{9em}}
                #3
            \end{tabular}
        };%
    }},
    zig zag to/.style={
        to path={(\tikztostart) -| ($(\tikztostart)!#1!(\tikztotarget)$) |- (\tikztotarget)}
    },
    zig zag to/.default=0.5,   
    one to one/.style={
        one-one, zig zag to
    },
    one to oone/.style={% One to Optional-one
        one-oone, zig zag to
    },
    oone to none/.style={% Optional-one to none
        oone-, zig zag to
    },
    oone to oone/.style={% Optional one to Optional-one
        oone-oone, zig zag to
    },
    one to many/.style={
        one-crow's foot, zig zag to,
    },
    one to omany/.style={
        one-omany, zig zag to
    },
    one to none/.style={
        one-, zig zag to
    },   
    many to many/.style={
        crow's foot-crow's foot, zig zag to
    }
}

==> macro.after.rollback.tex <==
\def\nbLib{94}
\def\nbLibStr{\np{\nbLib}\xspace}
\def\nbLibVersion{395}
\def\nbLibVersionStr{\np{\nbLibVersion}\xspace}
\def\nbLibCompiling{353}
\def\nbLibCompilingStr{\np{\nbLibCompiling}\xspace}
\def\nbLibDebloat{302}
\def\nbLibDebloatStr{\np{\nbLibDebloat}\xspace}
\def\nbTest{713659}
\def\nbTestStr{\np{\nbTest}\xspace}
\def\nbTestClient{74215}
\def\nbTestClientStr{\np{\nbTestClient}\xspace}
\def\nbFailingDebloatedTest{2645}
\def\nbFailingDebloatedTestStr{\np{\nbFailingDebloatedTest}\xspace}
\def\nbClientAll{2874}
\def\nbClientAllStr{\np{\nbClientAll}\xspace}
\def\nbClient{639}
\def\nbClientStr{\np{\nbClient}\xspace}
\def\nbFailDebloatClient{63}
\def\nbFailDebloatClientStr{\np{\nbFailDebloatClient}\xspace}
\def\nbValidatedDebloatedClient{492}
\def\nbValidatedDebloatedClientStr{\np{\nbValidatedDebloatedClient}\xspace}
\def\nbInvalidatedDebloatedClient{84}
\def\nbInvalidatedDebloatedClientStr{\np{\nbInvalidatedDebloatedClient}\xspace}
\def\meanCoverageLib{74.07}
\def\meanCoverageLibStr{\np{\meanCoverageLib}\xspace}
\def\medianCoverageLib{80.61}
\def\medianCoverageLibStr{\np{\medianCoverageLib}\xspace}
\def\meanCoverageClient{28.17}
\def\meanCoverageClientStr{\np{\meanCoverageClient}\xspace}
\def\medianCoverageClient{14.99}
\def\medianCoverageClientStr{\np{\medianCoverageClient}\xspace}
\def\nbLineLib{9676180}
\def\nbLineLibStr{\np{\nbLineLib}\xspace}
\def\nbLineClient{64162538}
\def\nbLineClientStr{\np{\nbLineClient}\xspace}
\def\executionTime{1 day, 23:34:13}
\def\debloatTime{21:22:46.091000}

% RQ1
\def\nbLibDebSuccessNum{309}
\def\nbLibNotCompile{40}
\def\nbLibCrash{29}
\def\nbLibTimeout{16}
\def\nbLibValidation{1}

\def\nbLibDebFailNum{4}


% RQ2
\def\nbLibPassTestNum{216}
\def\nbLibExcludedForTest{64}
\def\nbLibTestFailing{29}
\def\nbUniqueTestNum{328452}
\def\nbFailingTest{1296}
\def\nbErrorTest{321}


\FPeval{nbLibExecTestNum}{round(\nbLibPassTestNum + \nbLibTestFailing, 0)}
\FPeval{nbPassingTestNum}{round(\nbUniqueTestNum - \nbFailingTest, 0)}
\FPeval{nbFailureTest}{round(\nbFailingTest - \nbErrorTest, 0)}

% RQ3

\def\nbLibWithDependencies{76}
\def\nbDependencies{258}
\def\nbClasses{122199}
\def\nbMethods{677642}
\def\nbBloatedDependencies{50}
\def\nbBloatedClasses{77691}
\def\nbBloatedMethods{56804}
\def\nbDepClasses{47529}
\def\nbDepMethods{409148}
\def\nbBloatedDepClasses{31951}
\def\nbPreservedDepClasses{0}
\def\nbBloatedDepMethods{43430}

\FPeval{nbLibWithoutDependencies}{round(\nbLibPassTestNum - \nbLibWithDependencies, 0)}
\FPeval{nbNonBloatedDependencies}{round(\nbDependencies - \nbBloatedDependencies, 0)}

% RQ4 
\def\totalSize{1173820377}
\def\resourceSize{258848928}
\def\bytecodeSize{914971449}
\def\debloatedSize{620549107}
\def\debloatedMethodSize{13604786}
\def\preservedSize{0}
\def\internalTotal{259891628}

\FPeval{bloatedSize}{round(\debloatedSize + \debloatedMethodSize, 0)}
\FPeval{nonBloatedSize}{round(\bytecodeSize - \debloatedSize - \debloatedMethodSize, 0)}

% RQ5 & RQ6
\def\nbClient{1357}
\def\nbCoveringClient{1056}
\def\nbDynCoveringClient{276}
\def\nbStatCoveringClient{996}
\def\nbDifferentNbtest{5}
\def\nbFailingTestClient{54}
\def\nbFailingTestProject{40}
\def\nbClientTest{49580}
\def\nbClientFailure{1511}
\def\nbClientDebloatError{44}
\def\nbClientDebloatCompilationError{42}
\def\nbClientDebloatPluginError{2}
\def\nbClientDebloatOtherError{0}
\def\nbClientConsideredPreserved{977}
\def\nbClientWithPreserved{0}

\def\nbTotalProject{147991}
\def\nbTotalProjectStr{\np{\nbTotalProject}}

\FPeval{nbCientDebloatNoCompError}{round(\nbStatCoveringClient - \nbClientDebloatError, 0)}
\FPeval{nbClientDebloatNoTestFail}{round(\nbDynCoveringClient - \nbFailingTestClient, 0)}


\FPeval{nbFailingTestNum}{round(\nbUniqueTestNum - \nbPassingTestNum, 0)}
\FPeval{nbSuccessTestNum}{round(\nbPassingTestNum*100/\nbUniqueTestNum, 2)}
\def\nbLibPassTest{\np{\nbLibPassTestNum}\xspace}
\FPeval{nbLibFailTestNum}{round(\nbLibDebSuccessNum - \nbLibPassTestNum, 0)}
\FPeval{nbLibPassTestProportionNum}{round((\nbLibPassTestNum)*100/\nbLibDebSuccessNum, 2)}
\FPeval{debSuccessRate}{round(\nbLibDebSuccessNum*100/(\nbLibDebFailNum+\nbLibDebSuccessNum),2)}

\def\nbLibDebSuccess{\np{\nbLibDebSuccessNum}\xspace}
\def\nbLibDebFail{\np{\nbLibDebFailNum}\xspace}



% --------------------------
% Custom commands
% --------------------------

% Percentage number
\newcommand{\percSizeReduction}{$XXX\%$\@\xspace}
\newcommand{\percClassesReduction}{$XXX\%$\@\xspace}

% Common abbrev. are set as commands to ensure proper spacing after the dot
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{et al.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}
\newcommand{\mc}{Maven Central\@\xspace}
\newcommand{\latests}{\text{\texttt{LATESTS}\@\xspace}}
\newcommand{\pas}{\text{\texttt{P}\@\xspace}}
\newcommand{\act}{\text{\texttt{A}\@\xspace}}
\newcommand{\latest}{\text{$latest$\@\xspace}}
\newcommand{\notlatests}{\overline{\latests}}%% NOTE, it should be used in Math mode!

% tools
\newcommand\jdbl{{\textsf{JDBL}}\xspace}
\newcommand\proguard{{\sc Proguard}\xspace}
\newcommand\mv{{Maven}\xspace}
\newcommand\jar{\texttt{JAR}\xspace}

% comment commands for co-authors
\newcommand{\cesar}[1]{\mynote{C\'esar}{#1}}
\newcommand{\benoit}[1]{\mynote{Benoit}{#1}}
\newcommand{\nicolas}[1]{\mynote{Nicolas}{#1}}
\newcommand{\martin}[1]{\mynote{Martin}{#1}}
\newcommand{\thomas}[1]{\mynote{Thomas}{#1}} 
\newcommand{\todo}[1]{\mynote{TODO}{#1}} 
\newcommand{\modified}[1]{{\color{blue}#1}} 



==> macro.old.tex <==
\def\nbLib{94}
\def\nbLibStr{\np{\nbLib}\xspace}
\def\nbLibVersion{395}
\def\nbLibVersionStr{\np{\nbLibVersion}\xspace}
\def\nbLibCompiling{356}
\def\nbLibCompilingStr{\np{\nbLibCompiling}\xspace}
\def\nbTest{1728680}
\def\nbTestStr{\np{\nbTest}\xspace}
\def\nbTestClient{214177}
\def\nbTestClientStr{\np{\nbTestClient}\xspace}
\def\nbFailingDebloatedTest{2793}
\def\nbFailingDebloatedTestStr{\np{\nbFailingDebloatedTest}\xspace}
\def\nbClientAll{2876}
\def\nbClientAllStr{\np{\nbClientAll}\xspace}
\def\nbClient{1971}
\def\nbClientStr{\np{\nbClient}\xspace}
\def\nbFailDebloatClient{83}
\def\nbFailDebloatClientStr{\np{\nbFailDebloatClient}\xspace}
\def\nbValidatedDebloatedClient{1744}
\def\nbValidatedDebloatedClientStr{\np{\nbValidatedDebloatedClient}\xspace}
\def\nbInvalidatedDebloatedClient{144}
\def\nbInvalidatedDebloatedClientStr{\np{\nbInvalidatedDebloatedClient}\xspace}
\def\meanCoverageLib{76.45}
\def\meanCoverageLibStr{\np[\%]{\meanCoverageLib}\xspace}
\def\medianCoverageLib{84.32}
\def\medianCoverageLibStr{\np[\%]{\medianCoverageLib}\xspace}
\def\meanCoverageClient{31.3}
\def\meanCoverageClientStr{\np[\%]{\meanCoverageClient}\xspace}
\def\medianCoverageClient{20.79}
\def\medianCoverageClientStr{\np[\%]{\medianCoverageClient}\xspace}
\def\nbLineLib{24161481}
\def\nbLineLibStr{\np{\nbLineLib}\xspace}
\def\nbLineClient{91905172}
\def\nbLineClientStr{\np{\nbLineClient}\xspace}
\def\executionTime{4 days, 23:19:02}
\def\debloatTime{1 day and 21.5h}

% RQ1
\def\nbLibDebSuccessNum{309}
\def\nbLibNotCompile{39}
\def\nbLibCrash{27}
\def\nbLibTimeout{17}
\def\nbLibValidation{3}

\def\nbLibDebFailNum{4}


% RQ2
\def\nbLibPassTestNum{228}
\def\nbLibExcludedForTest{56}
\def\nbLibTestFailing{25}
\def\nbUniqueTestNum{353116}
\def\nbFailingTest{93}
\def\nbErrorTest{37}


\FPeval{nbLibExecTestNum}{round(\nbLibPassTestNum + \nbLibTestFailing, 0)}
\FPeval{nbPassingTestNum}{round(\nbUniqueTestNum - \nbFailingTest, 0)}
\FPeval{nbFailureTest}{round(\nbFailingTest - \nbErrorTest, 0)}

% RQ3

\def\nbLibWithDependencies{109}
\def\nbDependencies{283}
\def\nbClasses{126381}
\def\nbMethods{671856}
\def\nbBloatedDependencies{7}
\def\nbBloatedClasses{22213}
\def\nbBloatedMethods{63147}
\def\nbDepClasses{91374}
\def\nbDepMethods{380326}
\def\nbBloatedDepClasses{19811}
\def\nbPreservedDepClasses{8101}
\def\nbBloatedDepMethods{48553}

\FPeval{nbLibWithoutDependencies}{round(\nbLibPassTestNum - \nbLibWithDependencies, 0)}
\FPeval{nbNonBloatedDependencies}{round(\nbDependencies - \nbBloatedDependencies, 0)}

% RQ4 
\def\totalSize{997040347}
\def\resourceSize{207295589}
\def\bytecodeSize{789744758}
\def\debloatedSize{173649554}
\def\debloatedMethodSize{3070750}
\def\preservedSize{42886452}
\def\internalTotal{219910909}

\FPeval{nonBloatedSize}{round(\bytecodeSize - \debloatedSize - \debloatedMethodSize - \preservedSize, 0)}

% RQ5 & RQ6
\def\nbClient{1428}
\def\nbCoveringClient{1115}
\def\nbDynCoveringClient{306}
\def\nbStatCoveringClient{1052}
\def\nbDifferentNbtest{2}
\def\nbFailingTestClient{47}
\def\nbFailingTestProject{31}
\def\nbClientTest{51229}
\def\nbClientFailure{1375}
\def\nbClientDebloatError{17}
\def\nbClientDebloatCompilationError{16}
\def\nbClientDebloatPluginError{1}
\def\nbClientDebloatOtherError{0}
\def\nbClientConsideredPreserved{1022}
\def\nbClientWithPreserved{101}

\def\nbTotalProject{147991}
\def\nbTotalProjectStr{\np{\nbTotalProject}}

\FPeval{nbCientDebloatNoCompError}{round(\nbStatCoveringClient - \nbClientDebloatError, 0)}
\FPeval{nbClientDebloatNoTestFail}{round(\nbDynCoveringClient - \nbFailingTestClient, 0)}


\FPeval{nbFailingTestNum}{round(\nbUniqueTestNum - \nbPassingTestNum, 0)}
\FPeval{nbSuccessTestNum}{round(\nbPassingTestNum*100/\nbUniqueTestNum, 2)}
\def\nbLibPassTest{\np{\nbLibPassTestNum}\xspace}
\FPeval{nbLibFailTestNum}{round(\nbLibDebSuccessNum - \nbLibPassTestNum, 0)}
\FPeval{nbLibPassTestProportionNum}{round((\nbLibPassTestNum)*100/\nbLibDebSuccessNum, 2)}
\FPeval{debSuccessRate}{round(\nbLibDebSuccessNum*100/(\nbLibDebFailNum+\nbLibDebSuccessNum),2)}

\def\nbLibDebSuccess{\np{\nbLibDebSuccessNum}\xspace}
\def\nbLibDebFail{\np{\nbLibDebFailNum}\xspace}



% --------------------------
% Custom commands
% --------------------------

% Percentage number
\newcommand{\percSizeReduction}{$XXX\%$\@\xspace}
\newcommand{\percClassesReduction}{$XXX\%$\@\xspace}

% Common abbrev. are set as commands to ensure proper spacing after the dot
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{et al.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}
\newcommand{\mc}{Maven Central\@\xspace}
\newcommand{\latests}{\text{\texttt{LATESTS}\@\xspace}}
\newcommand{\pas}{\text{\texttt{P}\@\xspace}}
\newcommand{\act}{\text{\texttt{A}\@\xspace}}
\newcommand{\latest}{\text{$latest$\@\xspace}}
\newcommand{\notlatests}{\overline{\latests}}%% NOTE, it should be used in Math mode!

% tools
\newcommand\jdbl{{\textsf{JDBL}}\xspace}
\newcommand\proguard{{\sc Proguard}\xspace}
\newcommand\mv{{Maven}\xspace}
\newcommand\jar{\texttt{JAR}\xspace}

% comment commands for co-authors
\newcommand{\cesar}[1]{\mynote{C\'esar}{#1}}
\newcommand{\benoit}[1]{\mynote{Benoit}{#1}}
\newcommand{\nicolas}[1]{\mynote{Nicolas}{#1}}
\newcommand{\martin}[1]{\mynote{Martin}{#1}}
\newcommand{\thomas}[1]{\mynote{Thomas}{#1}} 
\newcommand{\todo}[1]{\mynote{TODO}{#1}} 
\newcommand{\modified}[1]{{\color{blue}#1}} 



==> macros_static.tex <==
\def\nbLib{94}
\def\nbLibStr{\np{\nbLib}\xspace}
\def\nbLibVersion{395}
\def\nbLibVersionStr{\np{\nbLibVersion}\xspace}
\def\nbLibCompiling{355}
\def\nbLibCompilingStr{\np{\nbLibCompiling}\xspace}
\def\nbLibDebloat{310}
\def\nbLibDebloatStr{\np{\nbLibDebloat}\xspace}
\def\nbTest{1725741}
\def\nbTestStr{\np{\nbTest}\xspace}
\def\nbTestClient{212448}
\def\nbTestClientStr{\np{\nbTestClient}\xspace}
\def\nbFailingDebloatedTest{4820}
\def\nbFailingDebloatedTestStr{\np{\nbFailingDebloatedTest}\xspace}
\def\nbClientAll{2874}
\def\nbClientAllStr{\np{\nbClientAll}\xspace}
\def\nbClient{1937}
\def\nbClientStr{\np{\nbClient}\xspace}
\def\nbFailDebloatClient{104}
\def\nbFailDebloatClientStr{\np{\nbFailDebloatClient}\xspace}
\def\nbValidatedDebloatedClient{1642}
\def\nbValidatedDebloatedClientStr{\np{\nbValidatedDebloatedClient}\xspace}
\def\nbInvalidatedDebloatedClient{191}
\def\nbInvalidatedDebloatedClientStr{\np{\nbInvalidatedDebloatedClient}\xspace}
\def\meanCoverageLib{74.17}
\def\meanCoverageLibStr{\np{\meanCoverageLib}\xspace}
\def\medianCoverageLib{80.83}
\def\medianCoverageLibStr{\np{\medianCoverageLib}\xspace}
\def\meanCoverageClient{31.07}
\def\meanCoverageClientStr{\np{\meanCoverageClient}\xspace}
\def\medianCoverageClient{20.13}
\def\medianCoverageClientStr{\np{\medianCoverageClient}\xspace}
\def\nbLineLib{10773047}
\def\nbLineLibStr{\np{\nbLineLib}\xspace}
\def\nbLineClient{138817982}
\def\nbLineClientStr{\np{\nbLineClient}\xspace}
\def\executionTime{4 days, 16:30:17}
\def\debloatTime{1 day, 11:16:52.641000}

% RQ1
\def\nbLibDebSuccessNum{310}
\def\nbLibNotCompile{40}
\def\nbLibCrash{27}
\def\nbLibTimeout{17}
\def\nbLibValidation{1}

\def\nbLibDebFailNum{4}


% RQ2
\def\nbLibPassTestNum{219}
\def\nbLibExcludedForTest{60}
\def\nbLibTestFailing{31}
\def\nbUniqueTestNum{334134}
\def\nbFailingTest{1459}
\def\nbErrorTest{486}


\FPeval{nbLibExecTestNum}{round(\nbLibPassTestNum + \nbLibTestFailing, 0)}
\FPeval{nbPassingTestNum}{round(\nbUniqueTestNum - \nbFailingTest, 0)}
\FPeval{nbFailureTest}{round(\nbFailingTest - \nbErrorTest, 0)}

% RQ3

\def\nbLibWithDependencies{74}
\def\nbDependencies{208}
\def\nbClasses{111660}
\def\nbMethods{590658}
\def\nbBloatedDependencies{37}
\def\nbBloatedClasses{47038}
\def\nbBloatedMethods{52345}
\def\nbDepClasses{36342}
\def\nbDepMethods{310008}
\def\nbBloatedDepClasses{15789}
\def\nbPreservedDepClasses{7406}
\def\nbBloatedDepMethods{38605}

\FPeval{nbLibWithoutDependencies}{round(\nbLibPassTestNum - \nbLibWithDependencies, 0)}
\FPeval{nbNonBloatedDependencies}{round(\nbDependencies - \nbBloatedDependencies, 0)}

% RQ4 
\def\totalSize{1174621775}
\def\resourceSize{258863663}
\def\bytecodeSize{915758112}
\def\debloatedSize{483715995}
\def\debloatedMethodSize{13604657}
\def\preservedSize{136862006}
\def\internalTotal{260143300}

\FPeval{bloatedSize}{round(\debloatedSize + \debloatedMethodSize, 0)}
\FPeval{nonBloatedSize}{round(\bytecodeSize - \debloatedSize - \debloatedMethodSize, 0)}

% RQ5 & RQ6
\def\nbClient{1384}
\def\nbCoveringClient{1072}
\def\nbDynCoveringClient{287}
\def\nbStatCoveringClient{1011}
\def\nbDifferentNbtest{5}
\def\nbFailingTestClient{54}
\def\nbFailingTestProject{40}
\def\nbClientTest{57997}
\def\nbClientFailure{1512}
\def\nbClientDebloatError{29}
\def\nbClientDebloatCompilationError{27}
\def\nbClientDebloatPluginError{1}
\def\nbClientDebloatOtherError{1}
\def\nbClientConsideredPreserved{992}
\def\nbClientWithPreserved{145}

\def\nbTotalProject{147991}
\def\nbTotalProjectStr{\np{\nbTotalProject}}

\FPeval{nbCientDebloatNoCompError}{round(\nbStatCoveringClient - \nbClientDebloatError, 0)}
\FPeval{nbClientDebloatNoTestFail}{round(\nbDynCoveringClient - \nbFailingTestClient, 0)}


\FPeval{nbFailingTestNum}{round(\nbUniqueTestNum - \nbPassingTestNum, 0)}
\FPeval{nbSuccessTestNum}{round(\nbPassingTestNum*100/\nbUniqueTestNum, 2)}
\def\nbLibPassTest{\np{\nbLibPassTestNum}\xspace}
\FPeval{nbLibFailTestNum}{round(\nbLibDebSuccessNum - \nbLibPassTestNum, 0)}
\FPeval{nbLibPassTestProportionNum}{round((\nbLibPassTestNum)*100/\nbLibDebSuccessNum, 2)}
\FPeval{debSuccessRate}{round(\nbLibDebSuccessNum*100/(\nbLibDebFailNum+\nbLibDebSuccessNum),2)}

\def\nbLibDebSuccess{\np{\nbLibDebSuccessNum}\xspace}
\def\nbLibDebFail{\np{\nbLibDebFailNum}\xspace}



% --------------------------
% Custom commands
% --------------------------

% Percentage number
\newcommand{\percSizeReduction}{$XXX\%$\@\xspace}
\newcommand{\percClassesReduction}{$XXX\%$\@\xspace}

% Common abbrev. are set as commands to ensure proper spacing after the dot
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{et al.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}
\newcommand{\mc}{Maven Central\@\xspace}
\newcommand{\latests}{\text{\texttt{LATESTS}\@\xspace}}
\newcommand{\pas}{\text{\texttt{P}\@\xspace}}
\newcommand{\act}{\text{\texttt{A}\@\xspace}}
\newcommand{\latest}{\text{$latest$\@\xspace}}
\newcommand{\notlatests}{\overline{\latests}}%% NOTE, it should be used in Math mode!

% tools
\newcommand\jdbl{{\textsf{JDBL}}\xspace}
\newcommand\proguard{{\sc Proguard}\xspace}
\newcommand\mv{{Maven}\xspace}
\newcommand\jar{\texttt{JAR}\xspace}

% comment commands for co-authors
\newcommand{\cesar}[1]{\mynote{C\'esar}{#1}}
\newcommand{\benoit}[1]{\mynote{Benoit}{#1}}
\newcommand{\nicolas}[1]{\mynote{Nicolas}{#1}}
\newcommand{\martin}[1]{\mynote{Martin}{#1}}
\newcommand{\thomas}[1]{\mynote{Thomas}{#1}} 
\newcommand{\todo}[1]{\mynote{TODO}{#1}} 
\newcommand{\modified}[1]{{\color{blue}#1}} 



==> old-intro.tex <==
Software systems have a natural tendency to grow over time, both in terms of size and complexity~\cite{Wirth1995, Holzmann2015, Quach2017}. 
A part of this growth comes with the addition of new features or different types of patches. 
Another part is due to the potentially useless code that  accumulates over time. This phenomenon, known as software bloat, is becoming more prevalent with the emergence of large software frameworks~\cite{Laperdrix2019,Koo2019,Rastogi2017}, and the widespread practice of code reuse~\cite{Zhong2019,Soto2020,Spinellis2021}.
Software debloating consists of automatically removing unnecessary code~\cite{Haas2020}. 
This task poses several challenges for code analysis and transformation: determine the bloated parts of the software system~\cite{Chen2017, Sharif2018, Qian2019}, remove these parts while keeping the integrity of the system, and produce a debloated version of the system that can still run and provide useful features.
In this context, the problem of effectively and safely debloating real-world applications remains a long-standing software engineering endeavor.

In this paper, we propose a novel software debloating technique for Java bytecode based on dynamic analysis.
When a library is executed with a given workload, our technique monitors the execution to capture which parts of the library's bytecode, as well as of its dependencies, are covered. 
We leverage the diversity of implementations of code coverage tools to collect accurate usage information at runtime.
We consolidate this runtime information with the JVM class loader logs to automatically generate debloated versions of Java libraries that compile and preserve their original behavior.

We notice that the collection of complete and  accurate coverage information is a key challenge when debloating Java applications based on code coverage. 
When the Java compiler translates source code to bytecode, it performs some irreversible code transformations, for example regarding \texttt{Enums} or implicit exceptions. 
Consequently, the existing coverage tools, which operate at the bytecode level, are prone to produce incomplete coverage results. 
As a consequence, debloating based on the coverage reports from a single coverage tool is likely to produce bytecode that is incorrect. 
Another part of the challenge relates to current coverage implementations, which do not collect information about third-party libraries.
We address both challenges through a novel blend of features provided by diverse code coverage tools, as well as an original extension to collect coverage in third-party libraries.

Our software debloating technique relies on consolidated coverage data collected at runtime.
It automatically transforms the bytecode and removes unnecessary code. 
Bytecode removal is performed on the library code as well as on the whole tree of third-party dependencies. 
To validate the usefulness of the debloated library, we build it with the same configuration as the original version.
This determines if the result of debloating is syntactically correct and if it preserves the behavior of the original software artifact.

We further validate the utility of the debloated Java artifacts by building client programs that use these artifacts as  third-party libraries. 
First, we check if the client compiles correctly with the debloated library. 
Then, we check if the client's test suite passes.
This is the first work in the debloating literature that assesses the utility of the debloated artifact with respect to its clients.

We implement our coverage-based debloating approach in a tool called \jdbl, the \underline{\textsc{J}}ava \underline{\textsc{D}}e\underline{\textsc{bl}}oater. 
\jdbl is tailored for Java projects that build with \mv to facilitate the integration with state-of-the-art build pipelines and the automation of the debloating procedure. 
We use \jdbl obtain debloated versions of \nbLibPassTestNum ~open-source Java libraries for a total 10M+ lines of code, which accounts for \np{\nbClasses} classes and \np{\nbDependencies} dependencies.
We assess the effectiveness of our technique to preserve both syntactic correctness and the original behavior of these libraries. 
We quantify the impact of coverage-based debloating with respect to the reduction of the libraries' size at three distinct granularity levels: number of removed methods, classes, and dependencies.
\jdbl finds that \ShowPercentage{\nbBloatedClasses}{\nbClasses} of classes in the libraries are bloated, which represents \np[\%]{68.3} of the libraries' bytecode, whereas the \ShowPercentage{\nbBloatedDependencies}{\nbDependencies} of dependencies can be completely removed.

We evaluate the utility of coverage-based debloating with respect to \np{\nbStatCoveringClient} ~clients that have at least one direct reference to the debloated library in their source code. 
Our experiments show that \ShowPercentage{\nbCientDebloatNoCompError}{\nbStatCoveringClient} of the clients successfully compile after replacing the library by its debloated version, and \ShowPercentage{\nbClientDebloatNoTestFail}{\nbDynCoveringClient} of clients which test suite covers at least one class of the library can successfully run their test suite, when using the debloated libraries.

\jdbl is the first debloating tool for Java that combines diverse coverage data sources with bytecode removal transformations, and validates the debloating results throughout the whole software build pipeline.
Unlike existing Java debloating techniques \cite{Bruce2020,Jiang2016}, our technique exploits the diversity of bytecode coverage tools to collect accurate and complete coverage information through the complete dependency tree.
The complete automation of the debloating procedure allows us to scale our experiments to large and diverse software projects, without any additional configuration. 
% We present the first debloating experiment that assesses the utility of bloated artifacts with respect to actual client usages.

In summary, this paper makes the following contributions:
\begin{itemize}[noitemsep]
	\item A practical bytecode debloating approach for Java artifacts based o the collection of complete coverage information from multiple sources.
	\item An open-source tool, \jdbl, which executes throughout the \mv build pipeline and automatically generates debloated versions of Java artifacts.
	\item The largest empirical study on software debloating performed on \nbLibVersionStr libraries, concerning code reduction at three granularity levels and using four different validation layers.
	\item A novel assessment of the impact of debloating for library clients, which exercises \np{\nbStatCoveringClient} clients of the \nbLibPassTest libraries that \jdbl successfully debloats. 
\end{itemize}

The rest of this paper is structured as follows: Section \ref{sec:background} presents a motivating example. 
Sections \ref{sec:third}, \ref{sec:methodology}, and \ref{sec:results} present the design and evaluation of our approach. 
Sections \ref{sec:threats} and \ref{sec:related} present the threats to validity and the related work. 

==> old-text.tex <==
%%%OLD ABSTRACT%%%
% Motivation:
To cope with the increasing demand of the markets, modern software development practices encourage the continuous addition of new functionalities. However, the average client may use only a small subset of the available features.
% Problem statement:
As a result, software applications become bloated, decreasing their overall performance, increasing the attack surface, and hindering usability.  
% Approach:
In this paper, we propose a novel approach to debloat software applications dynamically. We implement our approach in a tool, called \jdbl, that debloats compiled Java applications and its dependencies according to each individual user specifications.
% \jdbl integrates into the \mv building lifecycle.
% It can be used by clients to customize libraries in order to fit their particular needs.
% Results
We evaluate our approach by debloating \nbLib~real-world Java artifacts. The results show that \jdbl can reduce over \percSizeReduction of the bundled application size, decreasing the attack surface in \percClassesReduction, and releasing libraries that are more suitable for clients to reuse and extend. 
% Conclusion:
Moreover, by leveraging software diversity, our approach reduces vulnerabilities and increases security via moving target defense. Consequently, \jdbl is a practical and useful tool to automatically debloat Java applications.
%%%END OLD ABSTRACT%%%

%Previous works on software debloat have proposed different techniques, each of them tailored to a specific language. Significant efforts have been devoted to software debloat for C/C++ executable binaries. In this context, debloat starts from a program in which dependencies are compiled and linked statically~\cite{Quach2018,  Qian2019}. Debloat approaches for Java are scarce in the literature, and rely on static analysis to detect unreachable code~\cite{Jiang2018, Lafortune2004}. These techniques are challenged by the dynamic features of the language, such as type-induced dependencies~\cite{Sheng1998}, dynamic class loading~\cite{Li2018}, and reflection~\cite{Landman2017}. In addition, static analysis techniques are  conservative and do not remove \textit{unused code}~\cite{Foo2019, Lafortune2004}, \ie, the parts of an application that can be reached statically but are not executed at runtime, within a specific period, in a production environment.

%%%%%%coverage tools%%%

There are two different instrumentation modes in the coverage tools realm to distinguish the moment of when classes are being instrumented: 

\begin{itemize}
	\item \textit{off-line instrumentation.} The application classes are instrumented in a separate process in advance, before test execution.
	\item \textit{on-the-fly instrumentation.} The classes are instrumented while the class is loaded by the JVM, commonly using so called Java agents.
\end{itemize}

In JaCoCo, the mechanism of instrumentation is the same for both modes, and the output is the same as well. However, for our trace collection task, the off-line mode is the most effective because it does not impose any additional overhead during the execution of the workload. 


%\IEEEPARstart{S}{oftware} systems have a natural tendency to grow over time in terms of size and complexity~\cite{Holzmann2015, Quach2017}. The current development practices encourage developers to shorten releasing time intervals in order to provide more features that satisfy a broader number of clients. While this practice is intended to add more value to the final software product, most users actually need a minimal subset of the available functionalities. Therefore, software artifacts become increasingly bloated, which represents a waste in memory and resources that scales exponentially with every new release~\cite{Hibbs2009}. Besides, software bloat often leads to the unnecessary addition of exploitable functionalities, increasing vulnerabilities by amplifying the applications' attack surfaces~\cite{Xu2010, Bhattacharya2011}.

%In this context, software debloat techniques aim to mitigate this problem by providing mechanisms to reduce the artifacts' code size without compromising functionality, improving runtime performance, and decreasing attack surface. Unfortunately, most of the existing tools that are available for this purpose do not target large Java applications, focusing primarily on C/C++ executable binaries~\cite{Chen2017, Sharif2018, Qian2019}, and those that target Java rely on using static analysis approaches which are conservative and do not remove potentially unnecessary code (\eg,~\cite{Jiang2016, Jiang2018, Lafortune2004}. On the other hand, most previous works consider debloat as a post-processing step separated from development. No previous work has regarded the integration of debloat techniques as part of the artifacts' building lifecycle.


% \subsection{Trace-based debloat}

% \todo{this section is not done yet}
% Just like unnecessary source code increases the overall complexity of the software system and reduces developer productivity, additional binary instructions in libraries \todo{not lib, software} and its dependencies increase the complexity of client applications and impose potential maintenance risks. In this context, the debloat of unnecessary library functionalities is a suitable approach to tailor the library functionalities, to provide only the features needed by their clients. Based on this premise, two main challenges arise: $1$) from the perspective of library developers: How to integrate the debloat techniques into the building workflow, with a focus on the particular needs of its client?, and $2$) from the perspective of clients: How to make a distinction between the features that are required and the ones that should be removed in the library through the debloat process.

% The limitations of static analysis to determine which API members are used, in the context of dynamic features, forces the debloat to be rather conservative~\cite{Jiang2016, Jiang2018}. This motivates the usage of dynamic analysis for debloat, which allow us to precisely determine which parts of the program are necessary at run-time.

% The analysis of execution traces is a form of dynamic analysis useful for program comprehension tasks~\cite{Cornelissen2009}. Traditional tracing purposes include logging~\cite{Okanovi2016}, debugging~\cite{Han2012} and coverage analysis~\cite{Chen2018}. Recent works explore the monitoring of execution traces for program debloating~\cite{Vazquez2019, Foo2019}. 


 %https://www.jacoco.org/jacoco/trunk/doc/implementation.htm
 
 
 
 % RELATED WORK
 
 % Jiang \etal~\cite{Jiang2018} and Sharift \etal~\cite{Sharif2018} refer to software diversity as a potential benefit resulting from debloat. Our work advances software diversification to face the emergence of mono cultures in the reuse of third party application libraries~\cite{Baudry2015}. Our key novelty is the focus on debloat as as technique to improve the security of each application that reuses a library, while augmenting the diversity of versions of the reused libraries. This eventually leads to the emergence of diverse library versions, under the assumption that different applications do not reuse the same part of a given library. Yet, as far as we know, none of these works determines the impact of dynamic Java application specialization on the security of the applications nor studies in depth the diversity of library variants.
 
 %Unlike programming languages for which the dependencies are compiled and  statically~\cite{Quach2018, Lindholm2014}, the existence of modern dynamic features poses particular challenges for debloat Java applications, notably: type safety, dynamic class loading, and reflection. Java ensures type safety by enforcing type-induced dependencies~\cite{Sheng1998}. Classes in Java are dynamically compiled and loaded, and features such as dynamic class loading and reflection limit the ability of the compiler to determine which classes to load till the moment they are used~\cite{Landman2017}. In addition, there are other features in modern Java that allow developers to reuse, or even generate, classes at run-time without instantiate them~\cite{Li2018}, e.g., through plugged annotations, dynamic proxies, deserialization, or using the Java \texttt{Unsafe} API~\cite{Mastrangelo2015}.

% Notice that, although there are several levels of granularity at which the coverage trace can be obtained (\eg, classes, methods, branches, statements, instructions, etc.), \jdbl debloat on the granularity of dependencies, classes, and methods. The reason of this decision is that these are the fundamental  building blocks of modern Java projects, and hence the pieces that are more susceptible to be bloated. This level of coarse debloat granularity is often the most viable approach due to the large size of some Java projects. 

% Instead, we performed the experiments on the granularity of Java methods in real size Java systems with realistic test suites.Method-level granularity is often the viable solution due to the large system size. Fur- thermore, if we can demonstrate the weaknesses of the tools at this level, they are expected to be present at the lower levels of granularity as well.

%classpath tweaking

%https://www.jacoco.org/jacoco/trunk/doc/flow.html
%he control flow analysis and probe insertion strategy described in this document allows to efficiently record instruction and branch coverage. In total classes instrumented with JaCoCo increase their size by about 30\%. Due to the fact that probe execution does not require any method calls, only local instructions, the observed execution time overhead for instrumented applications typically is less than 10%.

% We notice that, despite of the union of all the information gathered from  different coverage tools, there are still some Java constructs that \jdbl  does not manage to cover, and which removal causes an incomplete debloat result.

% \todo{In order to overcome this problem, \jdbl enhances the dynamic usage information obtained from execution traces with static rules designed from our experience with the Java language.}
% \todo{The \texttt{Remove} phase starts with a static analysis step. Here, \jdbl collects a set of classes in the bytecode of the project under debloat that should not be removed (line \ref{line:algo:exc} in \autoref{algo:dynamic_debloat}).
% Specifically, \jdbl collects all classes with the following JVM bytecode access flags:  \texttt{ACC\_INTERFACE}, \texttt{ACC\_SYNTHETIC}, \texttt{ACC\_ANNOTATION}, \texttt{ACC\_ENUM}, and \texttt{ACC\_MODULE}. We also keep classes with the following bytecode constructs: primitive constants, user custom exceptions, and single-instruction methods. These language constructs are ubiquitous components of the Java language and are meant to support strong object oriented software design, with little or not procedural logic. While these constructs are important for humans to design and program in an object-oriented manner, they are useless for the machine to run the program. Consequently, they are not part of the executable code in the bytecode, and cannot be traced. Therefore, we need to adopt a conservative approach and conserve all of them, in order to produce a debloated program that is syntactically correct.}

% Due to the limitations of coverage tools discussed previously, and the information missing at compile-time, we use static analysis to avoid removing class files that cannot be traced dynamically at run-time. 


==> old_section2.tex <==
mv projects must include a particular build file, called \texttt{pom.xml}, which defines all the dependencies and build instructions necessary to produce an artifact.
Artifacts are typically packaged as \jar files.
These files are then deployed to a binary code repository to facilitate reuse by other projects.
In this work, the compiled \mv project is referred to as a \textit{library}, and the project that reuses the library is called a \textit{client}.

\begin{definition}
\textbf{Input space: }
The input space of a compiled \mv project is the set of all valid inputs for its public Application Programming Interface (API). 
\end{definition}

\mv projects provide API members, abstracting implementation details to facilitate external reuse. Libraries generally provide public API members for external reuse. However, there exist other dynamic reuse mechanisms that can be utilized by Java clients (\eg, through reflection, dynamic proxies, or the use of unsafe APIs).

\begin{definition}
\textbf{Workload: }
A workload is a set of valid inputs belonging to the input space of a compiled \mv project.
\end{definition}

Workloads are particularly useful for performing dynamic analysis.
For example, workloads are used to detect distinct execution paths in software applications, \eg, through profiling, and observability tasks. 
This type of technique aims at using monitoring tools to analyze how the application reacts to different workloads at runtime. 

\begin{definition}
\textbf{Execution trace: }
An execution trace is a sequence of calls between bytecode instructions in a compiled \mv project, obtained as a result of executing the project with a valid workload. 
\end{definition}

Given a valid workload for a project, one can obtain dynamic information about the program's behavior by collecting execution traces. 
We consider a trace as a sequence of calls, at the level of classes and methods, in compiled Java classes. 
A trace includes the bytecode of the project itself, as well as the classes and methods in third-party libraries. 

\begin{definition}
\textbf{Trace-based debloat: }
Given a project and an execution trace collected when running a specific workload on the project, trace-based debloat consists of removing the bytecode constructs that are not necessary to run the workload. Trace-based debloat takes a project and workload as input and produces a valid compiled Java project as output. The generated project, called the debloated project, is executable and has the same behavior as the original, modulo the workload.

Let $ \mathcal{P} $ be a program that contains a set of instructions $ \mathcal{S_P} $ and a workload that exercises a set $ \mathcal{F_P} $ of instructions, where $\mathcal{F_P} \subset \mathcal{S_P}$.
Trace-based debloat transforms $ \mathcal{P} $ into a \textit{correct} program $ \mathcal{P'} $, where $|\mathcal{S}_{P'}| < |\mathcal{S}_P|$ and $ \mathcal{P'} $ preserves the same behavior as $ \mathcal{P} $ when executing the workload.
\end{definition}

In the next section, we describe our main technical contribution in detail: an end-to-end pipeline for performing automatic trace-based debloat of Java programs, implemented in the \jdbl tool.

==> pom.tex <==
\begin{lstlisting}[style=Pom, xleftmargin=3.5ex, caption={Using \jdbl as a Maven plugin, which facilitates its execution and integration into the project's build life-cycle.}, label={lst:pom}]
<plugin>
   <groupId>se.kth.castor</groupId>
   <artifactId>jdbl-maven-plugin</artifactId>
   <version>1.0.0</version>
   <executions>
     <execution>
       <goals>
          <goal>trace-based-debloat</goal>
       </goals>
       </configuration>
     </execution>
   </executions>
</plugin>
\end{lstlisting}
\vspace{-40pt}

